Autonomous Robot for Disaster Mapping and Victim Localization

In response to the critical need for effective reconnaissance in disaster scenarios, this research article presents the design and implementation of a complete autonomous robot system using the Turtlebot3 with Robotic Operating System (ROS) Noetic. Upon deployment in closed, initially unknown environments, the system aims to generate a comprehensive map and identify any present 'victims' using AprilTags as stand-ins. We discuss our solution for search and rescue missions, while additionally exploring more advanced algorithms to improve search and rescue functionalities. We introduce a Cubature Kalman Filter to help reduce the mean squared error [m] for AprilTag localization and an information-theoretic exploration algorithm to expedite exploration in unknown environments. Just like turtles, our system takes it slow and steady, but when it's time to save the day, it moves at ninja-like speed! Despite Donatello's shell, he's no slowpoke - he zips through obstacles with the agility of a teenage mutant ninja turtle. So, hang on tight to your shells and get ready for a whirlwind of reconnaissance! Full pipeline code https://github.com/rzhao5659/MRProject/tree/main Exploration code https://github.com/rzhao5659/MRProject/tree/main

==> bibliography.tex <==
@book{sarkka2023bayesian,
  title={Bayesian filtering and smoothing},
  author={S{\"a}rkk{\"a}, Simo and Svensson, Lennart},
  volume={17},
  year={2023},
  publisher={Cambridge university press}
}


@inproceedings{ewfd,
  title={Expanding wavefront frontier detection: An approach for efficiently detecting frontier cells},
  author={Quin, Phillip and Alempijevic, Alen and Paul, Gavin and Liu, Dikai},
  booktitle={Australasian Conference on Robotics and Automation, ACRA},
  year={2014}
}

@inproceedings{fast-nbv,
  title={Fast sampling-based next-best-view exploration algorithm for a MAV},
  author={Respall, Victor Massagu{\'e} and Devitt, Dmitry and Fedorenko, Roman and Klimchik, Alexandr},
  booktitle={2021 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={89--95},
  year={2021},
  organization={IEEE}
}

@article{nbv2002,
author = {González-Baños, Héctor and Latombe, Jean-Claude},
year = {2002},
month = {10},
pages = {829-848},
title = {Navigation Strategies for Exploring Indoor Environments},
volume = {21},
journal = {I. J. Robotic Res.},
doi = {10.1177/027836402128964099}
}


@article{approaches-frontiers,
  title={Approaches for efficiently detecting frontier cells in robotics exploration},
  author={Quin, Phillip and Nguyen, Dac Dang Khoa and Vu, Thanh Long and Alempijevic, Alen and Paul, Gavin},
  journal={Frontiers in Robotics and AI},
  volume={8},
  pages={616470},
  year={2021},
  publisher={Frontiers Media SA}
}


@inproceedings{quin2014expanding,
  title={Expanding wavefront frontier detection: An approach for efficiently detecting frontier cells},
  author={Quin, Phillip and Alempijevic, Alen and Paul, Gavin and Liu, Dikai},
  booktitle={Australasian Conference on Robotics and Automation, ACRA},
  year={2014}
}

@online{Robotis,
    author = "Robotis",
    title = "Turtlebot3",
    url  = "https://emanual.robotis.com/docs/en/platform/turtlebot3/overview/",
    addendum = "(accessed: 03.09.2024)",
    keywords = "turtlebot3,setup"
}

@online{cameracalibration,
    author = "ROS",
    title = "How to Calibrate a Monocular Camera",
    url  = {http://wiki.ros.org//camera_calibration//Tutorials//MonocularCalibration},
    keywords = "turtlebot3,camera"
}

@online{ros,
  author = {{Stanford Artificial Intelligence Laboratory et al.}},
  title = {Robotic Operating System},
  url = {https://www.ros.org},
  version = {ROS Melodic Morenia},
  date = {2018-05-23},
}

@article{explore_lite,
  title={Map-merging for multi-robot system},
  author={H{\"o}rner, Ji{\v{r}}{\'\i}},
  year={2016},
  publisher={Univerzita Karlova, Matematicko-fyzik{\'a}ln{\'\i} fakulta}
}

@misc{move_base,
    title = {{ROS Wiki: move\_base}},
    howpublished = {\url{http://wiki.ros.org/move_base}},
    note = {Accessed: April 2024}
}

@inproceedings{gmapping,
    author = {Giorgio Grisetti and Cyrill Stachniss and Wolfram Burgard},
    title = {{Improved Techniques for Grid Mapping With Rao-Blackwellized Particle Filters}},
    booktitle = {IEEE International Conference on Robotics and Automation (ICRA)},
    year = {2007},
    pages = {3928--3933},
    doi = {10.1109/ROBOT.2007.364030}
}

@inproceedings{apriltag_ros,
  title={AprilTag 2: Efficient and robust fiducial detection},
  author={Wang, John and Olson, Edwin},
  booktitle={2016 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={4193--4198},
  year={2016},
  organization={IEEE}
}

@article{gazebo,
  title={Design and implementation of the player/stage/gazebo project},
  author={Koenig, Nathan and Howard, Andrew},
  journal={Proceedings of the 2004 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS 2004)},
  pages={2149--2154},
  year={2004},
  organization={IEEE}
}
